Object-oriented Neural Programming (OONP) for Document Understanding

We propose Object-oriented Neural Programming (OONP), a framework for semantically parsing documents in specific domains. Basically, OONP reads a document and parses it into a predesigned object-oriented data structure (referred to as ontology in this paper) that reflects the domain-specific semantics of the document. An OONP parser models semantic parsing as a decision process: a neural net-based Reader sequentially goes through the document, and during the process it builds and updates an intermediate ontology to summarize its partial understanding of the text it covers. OONP supports a rich family of operations (both symbolic and differentiable) for composing the ontology, and a big variety of forms (both symbolic and differentiable) for representing the state and the document. An OONP parser can be trained with supervision of different forms and strength, including supervised learning (SL) , reinforcement learning (RL) and hybrid of the two. Our experiments on both synthetic and real-world document parsing tasks have shown that OONP can learn to handle fairly complicated ontology with training data of modest sizes.

==> e2.tex <==
\subsection{Task-II: Parsing Police Report}
\subsubsection{Data \&  task}
We implement \OONP for parsing  Chinese police report (brief description of criminal cases written by policeman), as illustrated in the left panel of Figure  \ref{fig:task-example}.   We consider a corpus of 5,500 cases with a variety of crime categories,  including theft, robbery, drug dealing and others.  The ontology we designed for this task mainly consists of a number of  \poos and \ioos connected through a \eoo with several types of relations, as illustrated in the right panel of Figure  \ref{fig:task-example}.  A \poo has three internal properties: \name (string),  \gender (categorical) and \age (number), and two types of external links (\suspect and \victimx) to an \eoox.  An \ioo has three internal properties: \name (string), \quantity (string) and \valuee (string), and six types of external links  (\texttt{stolen}, \texttt{drug}, \texttt{robbed}, \texttt{swindled}, \texttt{damaged}, and \texttt{other}) to an \eoox.
%\newpage
\begin{figure}[h!]
	\centering
	\includegraphics[width=0.85\linewidth]{image/taskExample2.png}
	%\vspace{-100pt}
	\caption{An example of police report and its ontology.}\label{fig:task-example}
	%\vspace{-2mm}
\end{figure}


\subsubsection{Implementation details}

 The \OONP model is designed to generate ontology as illustrated in Figure  \ref{fig:task-example}  through a decision process with actions in  Table \ref{tab:actions-Police2}.   As pre-processing, we performed regular NER with third party algorithm (therefore not part of the learning) and simple rule-based extraction to yield the symbolic part of \inline as shown in Figure \ref{fig:inlineExample-task2}.  For the distributed part of \inlinex, we used dilated CNN with different choices of depth and kernel size~\cite{dilatedCNN},  all of which will be jointly learned during training.  In making the \newassign decision,  \Reader considers matching of two structured objects, as well as the hints from the symbolic part of \inline as features, as pictorially illustrated in Figure \ref{fig:richStructure}.  In updating objects with its string-type properties (e.g., \name for a \poo ), we use Copy-Paste strategy for extracted string (whose NER tag already specifies which property in  an object  it goes to) as \Reader sees it.  For undetermined category properties in existed objects,  \pn will determine the object to update (an \newassign action without \neww option), its property to update (an \updatewhat action), and the updating operation (an \updatetowhat action) at milestones of the decision process , e.g., when reaching an punctuation. For this task, since all the relations are between the single by-default \eoo and other objects,  the relations can be reduced to category-type properties of the corresponding objects in practice.  For category-type properties,  we cannot recover  \newassign   and \updatewhat actions from the label (the final ontology), so we resort RL for learning to determine that part, which is mixed with the supervised learning for \updatetowhat and other actions for string-type properties.  An example of a complete decision process can be found in Figure \ref{fig:fullEpisode-E2}. 
 


\begin{table*}[h!]
	\centering
	\resizebox{1\linewidth}{!}{
		\begin{tabular}{|ll|}
			\hline
			\textbf{Action} & \textbf{Description}       \\
			\hline\hline
			\texttt{NewObject($c$)} & New an object of class-$c$.  \\
			\texttt{AssignObject($c,k$)}      & Assign the current information to existed object $(c,k)$ \\
			\texttt{UpdateObject($c,k$).Name}      & Set the name of object-$(c,k)$ with the extracted string.\\
			\texttt{UpdateObject($\pppx,k$).Gender}      & Set the name of a \poo indexed $k$ with the extracted string.\\
			\texttt{UpdateObject($\iiix,k$).Quantity}  & Set the quantity of an \ioo indexed $k$  with the extracted string.\\
			\texttt{UpdateObject($\iiix,k$).Value}  & Set the value of an  \ioo indexed $k$ with the extracted string.\\
			\texttt{UpdateObject($\eeex,1$).Items.x} & Set the link between the \eoo and an \ioox, where  
			 \texttt{x} $\in$\{\texttt{stolen}, \\& \texttt{drug}, \texttt{robbed}, \texttt{swindled}, \texttt{damaged}, \texttt{other}\}\\
			\texttt{UpdateObject($\eeex,1$).Persons.x} & Set the link between the \eoo and an \poox, 
			                                                        and \texttt{x} $\in$\{\victimx, \\& \suspectx \}\\
			\hline
		\end{tabular}
	}\vspace{-2mm}
	\caption{Actions for parsing police report.}\label{tab:actions-Police2}
	\vspace{-2mm}
\end{table*}




\subsubsection{Results \& discussion}

We use 4,500 cases for training, 500 for validation an held-out 500 for test. For evaluation, we compare the {\color{red} XXXXXXXX } 

%{\LARGE The table of results!!}
\begin{table*}[!hbtp]
	\centering
	\resizebox{1\linewidth}{!}{
		\begin{tabular}{|l|l|l|l|l|l|l|}
			\hline
			\multirow{2}{*}{\textbf{Model Variant}} & \multicolumn{3}{|c|}{\textbf{Object Assign Accu}} & \multicolumn{3}{|c|}{\textbf{Object Type Accu}}\\ \cline{2-7}
			&train&dev&test&train&dev&test\\
			\hline\hline
			\texttt{naive BiGRU} &xx&xx&xx&xx&xx&xx\\
			\texttt{OONP(base)[1]} &xx&xx&xx&xx&xx&xx \\
			\texttt{OONP(lcs feature)[2]} &98\%&91.9\%&xx&97\%&85.6\%&xx\\
			\texttt{OONP(slot mems)[3]}  &xx&xx&xx&xx&xx&xx\\
			\texttt{OONP(RL obj type)[4]} &xx&xx&xx&xx&xx&xx\\
			\texttt{OONP(obj type feature)[5]} &xx&xx&xx&xx&xx&xx\\
			\texttt{OONP([2-4])} &xx&xx&xx&xx&xx&xx\\
			\hline
		\end{tabular}
	}\vspace{-2mm}
	\caption{The table of results.(symbolic lcs rule;and other variants)}\label{tab:results}
	\vspace{-2mm}
\end{table*}
\newpage
An example
Results are given in table 1.
The results showing that combining with symbolic rule features is amazing. Structured objects is amazing. RL could judge at the right time.

\begin{figure}[h!]
	\centering
	\includegraphics[width=1\linewidth]{image/runningExample.png}
	%\vspace{-100pt}
	\caption{An example of full episode of parsing police report.}\label{fig:fullEpisode-E2}
	%\vspace{-2mm}
\end{figure}






